Circuits via topoi

Leveraging topos theory a semantics can be given to sequential circuits where time-sensitive gates, such as unit delay, are treated uniformly with combinational gates. Both kinds of gates are functions in a particular topos: the topos of presheaves over the natural ordering of $\mathbb{N}$. This is used to show that sequential circuits validate the equational theory of traced categories.

==> style.tex <==
% J'utilise un fichier .tex pour régler le style de la classe memoir
% parce que ça semble la meilleure façon.


%%% heading for @ purposes
\makeatletter

%%% Numérotation

\setsecnumdepth{subsection}
\maxsecnumdepth{subsection}

%%% Configuration du & pour qu'il soit en italique

\let\oldampersand\&
\renewcommand*\&{{\itshape\oldampersand}}

%%% Configuration de la police : Palatino + Text Numerals
% quelque soit le choix de police, pour une meilleur lecture
% à l'écran, \usagepackage{fontenc}[T1] est recommandé
\renewcommand{\rmdefault}{pplj}
\let\cmoldstylenums\oldstylenums %text numerals in Computer Modern
\renewcommand{\oldstylenums}[1]{%
  {\fontfamily{pplj}\selectfont #1}}

%%% Footer for @ purposes
\makeatother

